3x2: 3D Object Part Segmentation by 2D Semantic Correspondences

3D object part segmentation is essential in computer vision applications. While substantial progress has been made in 2D object part segmentation, the 3D counterpart has received less attention, in part due to the scarcity of annotated 3D datasets, which are expensive to collect. In this work, we propose to leverage a few annotated 3D shapes or richly annotated 2D datasets to perform 3D object part segmentation. We present our novel approach, termed 3-By-2 that achieves SOTA performance on different benchmarks with various granularity levels. By using features from pretrained foundation models and exploiting semantic and geometric correspondences, we are able to overcome the challenges of limited 3D annotations. Our approach leverages available 2D labels, enabling effective 3D object part segmentation. Our method 3-By-2 can accommodate various part taxonomies and granularities, demonstrating interesting part label transfer ability across different object categories. Project website: \url{https://ngailapdi.github.io/projects/3by2/}.

==> tables/affordancenet_rebuttal.tex <==
\begin{table}[t]

\begin{center}


\begingroup
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\caption{Ablation of the non-overlapping mask generation module.}
% \vspace{-10pt}
\scalebox{0.9}{


% \begin{table*}[h]
% \centering
% \caption{PartNetE}
\begin{tabular}{l|cc}
Category & mIoU \\
\hline
 Hat & 0.880 \\
\hline
Earphone & 0.654

\end{tabular}

\label{tab:afn_ret}
%\caption{Characteristics of different single-view 3D shape reconstruction methods. }
}
\endgroup

\end{center}
\end{table}

==> tables/compare.tex <==
\begin{table}[t]
\begin{center}


\begingroup
\setlength{\tabcolsep}{4pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\caption{\textbf{Properties of SOTA low-shot 3D part segmentation methods.} Compared to other methods, our approach demonstrates strong capability with flexible input signals.}
\scalebox{0.7}{
\begin{tabular}{l|c|c|c|c|c}
\diagbox[width=10em]{Properties}{Methods} & \begin{tabular}{@{}c@{}} PartSLIP\vspace{-3pt}\\ \cite{liu2023partslip} \end{tabular}  & \begin{tabular}{@{}c@{}} SATR\vspace{-3pt}\\ \cite{abdelreheem2023satr} \end{tabular} & \begin{tabular}{@{}c@{}} MvDeCor\vspace{-3pt}\\ \cite{sharma2022mvdecor} \end{tabular}&  \begin{tabular}{@{}c@{}} PointCLIPv2\vspace{-3pt}\\ \cite{zhu2023pointclip} \end{tabular}& \begin{tabular}{@{}c@{}} 3-By-2\vspace{-3pt}\\ (Ours) \end{tabular} \\
\hline
Zero-shot                  & \cmark & \cmark & \xmark  & \cmark   & \cmark  \\    
Few-shot       & \cmark & \xmark & \cmark  & \cmark   & \cmark  \\
Training-free                   & \xmark & \cmark & \xmark  & \xmark  & \cmark \\
Language-free Input   & \xmark & \xmark & \cmark & \xmark  & \cmark    \\
Without Segmented 3D Priors              & \xmark & \xmark & \xmark   & \cmark  & \cmark 
\end{tabular}
\label{tab:compare}
%\caption{Characteristics of different single-view 3D shape reconstruction methods. }
}
\endgroup

\vspace{-20pt}
\end{center}

\end{table}
